Level Lines of Gaussian Free Field II: Whole-Plane GFF

We study the level lines of GFF starting from interior points. We show that the level line of GFF starting from an interior point turns out to be a sequence of level loops. The sequence of level loops satisfies "target-independent" property. All sequences of level loops starting from interior points give a tree-structure of the plane. We also introduce the continuum exploration process of GFF starting from interior. The continuum exploration process of whole-plane GFF satisfies "reversibility".

==> tex/wholeplane_cle4_construction.tex <==
In this section, we will explain the construction and some properties of whole-plane $\CLE_4$ and complete the proof of Theorem \ref{thm::wholeplane_cle4_reversibility}. In fact, all conclusions in this section about whole-plane $\CLE_4$ are explained in \cite{KemppainenWernerNestedSimpleCLERiemannSphere}, and we will explain how to obtain these properties in the current setting.  

As introduced in Section \ref{subsec::growing_cle4}, $\CLE$ in simply connected domain $D\neq\C$ is a random countable collection of simple loops in $D$ that are disjoint and non-nested. It is natural to define nested $\CLE$ in $D$ from non-nested $\CLE$s in an iterative i.i.d way: Sample first non-nested $\CLE$ in $D$, and then sample independent $\CLE$s in the inside of each loop in the first generation, and iterate. This defines a nested $\CLE$ in $D$ which is a collection of disjoint simple loops, but, for each fixed $z\in D$, there are infinitely many loops that surround $z$. From nested $\CLE$, there is a natural version of $\CLE$ defined in the whole-plane (see \cite{KemppainenWernerNestedSimpleCLERiemannSphere, MillerWatsonWilsonExtremeNestingCLE}) obtained via a limiting procedure: one considers a nested $\CLE$ in $\C\cup\{\infty\}\setminus \eps\U$ and the whole-plane nested $\CLE$ is the limit object as $\eps$ goes to zero. 

In Section \ref{subsec::gff_discrete_continuum}, we introduced the upward continuum exploration process of $\GFF$ on $\U$, and we explained that the collection of all clockwise loops in the upward continuum exploration processes of $\GFF$ targeted at all points in $\U$ is a (non-nested) $\CLE_4$: Proposition \ref{prop::upward_continuum_cle4}. In Section \ref{subsec::gff_alternate_continuum}, we introduced the alternating continuum exploration process of $\GFF$ on $\U$ which is generated in an iterative i.i.d way. Therefore, the corresponding loops in the alternating continuum exploration processes targeted at all points in $\U$ gives a nested $\CLE_4$: Proposition \ref{prop::alternate_continuum_cle4_nested}. From the coupling between whole-plane $\GFF$ and the alternating continuum exploration process given in Theorem \ref{thm::interior_continuum_coupling}, we obtain a coupling between $\GFF$ and whole-plane nested $\CLE_4$.

\begin{proposition}
Suppose that $h$ is a whole-plane $\GFF$ modulo a global additive constant in $\R$.
\begin{enumerate}
\item [(1)] For any two points $z,w\in\C\cup\{\infty\}$, let $(L_u, u\in\R)$ be the alternating continuum exploration process of $h$ starting from $z$ targeted at $w$ where $(u_j, j\in\Z)$ is the sequence of transition times. Then the collection of loops $(\gamma^{z\to w}_j:=L_{u_j}, j\in\Z)$ has the same law as the sequence of loops in whole-plane nested $\CLE_4$ that disconnects $z$ from $w$. We call $(\gamma^{z\to w}_j, j\in\Z)$ the \textbf{sequence of transition loops} of $h$ starting from $z$ targeted at $w$ and denote its law by $\CLE_4(z\to w)$.
\item [(2)] For any $z\in\C\cup\{\infty\}$, consider the sequences of transition loops of $h$ starting from $z$ targeted at all points in $\C$: $((\gamma^{z\to w}_j, j\in\Z), w\in\C)$. The collection of loops $\{\gamma^{z\to w}_j: j\in\Z, w\in\C\}$ has the same law as whole-plane nested $\CLE_4$. We denote its law by $\CLE_4(z\to\C)$.
\end{enumerate}
\end{proposition}  

The conformal invariance of whole-plane $\GFF$ would imply the conformal invariance of whole-plane nested $\CLE_4$; and the properties of the alternating continuum exploration process in Theorems \ref{thm::interior_continuum_interacting_commontarget} and \ref{thm::interior_continuum_interacting_commonstart} would imply the corresponding properties of whole-plane nested $\CLE_4$.

\begin{proposition}\label{prop::wholeplane_cle4_properties}
Suppose that $h$ is a whole-plane $\GFF$ modulo a global additive constant in $\R$.
\begin{enumerate}
\item [(1)] Whole-plane nested $\CLE_4$ satisfies conformal invariance: for any M\"obius transformation $\phi$ of the Riemann sphere, the collection of the image of the loops in $\CLE_4(z\to w)$ under $\phi$ has the same law as $\CLE_4(\phi(z)\to\phi(w))$ for any $z,w\in\C\cup\{\infty\}$; the collection of the image of the loops in $\CLE_4(z\to\C)$ under $\phi$ has the same law as $\CLE_4(\phi(z)\to\C)$ for any $z\in\C\cup\{\infty\}$.

\item [(2)] Fix two points $z_1, z_2\in\C$. For $i=1,2$, let $(\gamma^{z_i\to\infty}_j, j\in\Z)$ be the sequence of transition loops of $h$ starting from $z_i$ targeted at $\infty$. Define
\[N_1=\min\{j: \gamma^{z_1\to\infty}_j\text{ disconnects }z_2\text{ from }\infty\},\quad N_2=\min\{j: \gamma^{z_2\to\infty}_j\text{ disconnects }z_1\text{ from }\infty\}.\]
Then, almost surely, the two sequences of loops $(\gamma^{z_1\to\infty}_j, j\ge N_1)$ and $(\gamma^{z_2\to\infty}_j, j\ge N_2)$ coincide.

\item [(3)] Fix three points $z, w_1, w_2\in\C\cup\{\infty\}$. For $i=1,2$, let $(\gamma^{z\to w_i}_j, j\in\Z)$ be the sequence of transition loops of $h$ starting from $z$ targeted at $w_i$ and denote by $U_n^{w_i}$ the connected component of $\C\cup\{\infty\}\setminus\gamma^{z\to w_i}_n$ that contains $w_i$. Then there exists a number $N$ such that 
\[\gamma^{z\to w_1}_n=\gamma^{z\to w_2}_n,\quad \text{for }n<N;\quad U_N^{w_1}\cap U_N^{w_2}=\emptyset.\]
In particular, this implies the target-independence of whole-plane nested $\CLE_4$: $\CLE_4(z\to w_1)$ and $\CLE_4(z\to w_2)$ have the same law on the sequence of loops starting from $z$ stopped at the first time that $w_1$ and $w_2$ are disconnected. 

\end{enumerate}
\end{proposition}


==> tex/wholeplane_cle4_reversibility.tex <==
To explain the conclusion in Theorem \ref{thm::wholeplane_cle4_reversibility}, we need to briefly recall some features of $\CLE$ in the annulus and we refer to \cite{SheffieldWatsonWuSimpleCLEDoubly} for details and proofs. 
Suppose that $A$ is an annulus. The \textbf{non-nested $\CLE$ in the annulus} $A$ is the collection of the outer boundaries of outermost clusters of the Brownian loop soup in $A$ conditioned on the event that there is no cluster that disconnects the two connected components of $\partial A$ (\cite[Section 3.1]{SheffieldWatsonWuSimpleCLEDoubly}). $\CLE$ in the annulus is conformal invariant:

\begin{lemma}\label{lem::cle_annulus_conformalinvariance}
Fix an annulus $A$ which is invariant under inversion. Then $\CLE$ in the annulus $A$ is invariant under inversion.
\end{lemma}
\begin{proof}
\cite[Proposition 3.2]{SheffieldWatsonWuSimpleCLEDoubly}.
\end{proof}

The relation between non-nested $\CLE$ in the annulus and non-nested $\CLE$ in the unit disc is described through the following lemma. 

\begin{lemma}\label{lem::cle_annulus_unitdisc}
Suppose that $\Gamma$ is a non-nested $\CLE$ in $\U$ and that $L(0)$ is the loop in $\Gamma$ that surrounds the origin. Define $A$ to be the annulus lying between $\partial\U$ and $L(0)$:
\[A=\U\setminus\overline{\inte{L(0)}}.\]
Then, given $A$, the conditional law of the loops in $\Gamma$ that stay in $A$ is the same as $\CLE$ in the annulus $A$.
\end{lemma}
\begin{proof}
\cite[Proposition 3.5]{SheffieldWatsonWuSimpleCLEDoubly}.
\end{proof}

Define \textbf{nested $\CLE$ in the annulus} $A$ in the following way: Sample first non-nested $\CLE$ $\Gamma_A$ in $A$, and then sample independent nested $\CLE$s in the inside of each loop of $\Gamma_A$. 

Consider a whole-plane nested $\CLE_4(0\to\C)$, we have the following observations.
\begin{enumerate}
\item [(a)] By Proposition \ref{prop::wholeplane_cle4_properties} Item (1), we know that $\CLE_4(0\to\C)$ is invariant under any M\"obius transformation $\phi$ of the Riemann sphere such that $\phi(0)=0$.  
\item [(b)] Suppose that $(\gamma_j, j\in\Z)$ is a sequence of loops with law $\CLE_4(0\to\infty)$. Define $A_j$ to be the annulus lying between $\gamma_j$ and $\gamma_{j+1}$:
\[A_j=\ext(\gamma_j)\setminus\overline{\ext(\gamma_{j+1})}.\]
Given $(\gamma_j,  j\in\Z)$, for each $j$, sample independent nested $\CLE_4$ in the annulus $A_j$. Then the obtained collection of loops (the loops $(\gamma_j, j\in\Z)$ and the loops inside each annulus $A_j$) has the same law as $\CLE_4(0\to\C)$ by Lemma \ref{lem::cle_annulus_unitdisc}.
\item [(c)] By Lemma \ref{lem::cle_annulus_conformalinvariance}, we know that the nested $\CLE_4$ in the annulus is invariant under inversion. 
\end{enumerate}
Combining these three facts, to prove Theorem \ref{thm::wholeplane_cle4_reversibility}, it is sufficient to show that $\CLE_4(0\to\infty)$ is invariant under inversion. In other words, the proof of Theorem \ref{thm::wholeplane_cle4_reversibility} will be completed by proving the following proposition.

\begin{proposition}
The law $\CLE_4(0\to\infty)$ is the same as $\CLE_4(\infty\to 0)$.
\end{proposition}

\begin{proof}
Suppose that $(\gamma_j, j\in\Z)$ is a sequence of loops with law $\CLE_4(0\to\infty)$. For each $j$, define $A_j$ to be the annulus lying between $\gamma_j$ and $\gamma_{j+1}$. Define the intensity measure $\mu_A$ in the following way: for each measurable set $\LA$ of annuli, set 
\[\mu_A[\LA]=\E[\#\{j: A_j\in\LA\}].\]

\textit{First}, combining Lemmas \ref{lem::growing_cle4_operation1}, \ref{lem::growing_cle4_operation2} with Corollary \ref{cor::intensitymeasures_reversibility}, we know that $\mu_A$ is invariant under inversion.
\medbreak
Consider the sequence of annuli $(A_j, j\in\Z)$, almost surely, there exists exactly one annulus that contains the point $1$. We reindex the loops by $1/2+\Z$ such that $1$ is between the two loops $\gamma_{-1/2}$ and $\gamma_{1/2}$. 

\textit{Second}, we explain that the law of the pair $(\gamma_{-1/2}, \gamma_{1/2})$ is invariant under inversion. Denote by $\mu_{A,1}$ the measure of $\mu_A$ restricted to the annuli that contain $1$. The measure $\mu_{A,1}$ is a probability measure. We have the following observations.
\begin{enumerate}
\item [(a)] By the first step, we know that $\mu_A$ is invariant under inversion, thus $\mu_{A,1}$ is also invariant under inversion.
\item [(b)] The law of the pair $(\gamma_{-1/2}, \gamma_{1/2})$ is the same as the law of the two connected components of the boundary of the annulus with law $\mu_{A,1}$.
\end{enumerate}  
Combining these two facts, we have that the law of the pair $(\gamma_{-1/2}, \gamma_{1/2})$ is invariant under inversion.
\medbreak
\textit{Finally}, we explain that the law of the sequence $(\gamma_{-1/2-n},..., \gamma_{-1/2}, \gamma_{1/2}, ..., \gamma_{1/2+n})$ is invariant under inversion for any $n\ge 1$. In fact, the similar argument for the case $n=0$ also works here. Define the measure on the set of successive $(2n+1)$-annuli such that $1$ is in the inside of the middle annulus, then this measure is also invariant under inversion. This implies that the law of the sequence $(\gamma_{-1/2-n},..., \gamma_{-1/2}, \gamma_{1/2}, ..., \gamma_{1/2+n})$ is invariant under inversion. This completes the proof. 
\end{proof}
